A Study on Deep CNN Structures for Defect Detection From Laser Ultrasonic Visualization Testing Images

The importance of ultrasonic nondestructive testing has been increasing in recent years, and there are high expectations for the potential of laser ultrasonic visualization testing, which combines laser ultrasonic testing with scattered wave visualization technology. Even if scattered waves are visualized, inspectors still need to carefully inspect the images. To automate this, this paper proposes a deep neural network for automatic defect detection and localization in LUVT images. To explore the structure of a neural network suitable to this task, we compared the LUVT image analysis problem with the generic object detection problem. Numerical experiments using real-world data from a SUS304 flat plate showed that the proposed method is more effective than the general object detection model in terms of prediction performance. We also show that the computational time required for prediction is faster than that of the general object detection model.

==> jiii2023miya-draft-000-abst.tex <==
\title{A Study on Deep CNN Structures for Defect Detection From Laser Ultrasonic
Visualization Testing Images}
%
\endtitle{A Study on Deep CNN Structures for Defect Detection From Laser Ultrasonic Visualization Testing Images}

\author{Miya NAKAJIMA\thanks{Member of JSCE, Graduate Student, Graduate School of Science and Technology, Gunma University \\(Tenjin 1-5-1, Kiryu, Gunma 376-8515, Japan)\email{t221d064@gunma-u.ac.jp} (Corresponding author)}・ % \email{t221d064@gunma-u.ac.jp}}・
Takahiro SAITOH\thanks{Member of JSCE, Associate Professor, Graduate School of Science and Technology, Gunma University \\(Tenjin 1-5-1, Kiryu, Gunma 376-8515, Japan)}・
Tsuyoshi KATO\thanks{Professor, Faculty of Informatics, Gunma University\\(Aramaki 4-2, Maebashi, Gunma 371-8510, Japan)}}

\abstract{The importance of ultrasonic nondestructive testing has been increasing in recent years, and there are high expectations for the potential of laser ultrasonic visualization testing, which combines laser ultrasonic testing with scattered wave visualization technology. Even if scattered waves are visualized, inspectors still need to carefully inspect the images. To automate this, this paper proposes a deep neural network for automatic defect detection and localization in LUVT images. To explore the structure of a neural network suitable to this task, we compared the LUVT image analysis problem with the generic object detection problem. Numerical experiments using real-world data from a SUS304 flat plate showed that the proposed method is more effective than the general object detection model in terms of prediction performance. We also show that the computational time required for prediction is faster than that of the general object detection model.}

\keywords{Non-destructive testing, laser ultrasonic visualization testing, deep neural network, object detection, defect detection, defect localization}

